Data-driven Energy Efficiency Modelling in Large-scale Networks: An Expert Knowledge and ML-based Approach

The energy consumption of mobile networks poses a critical challenge. Mitigating this concern necessitates the deployment and optimization of network energy-saving solutions, such as carrier shutdown, to dynamically manage network resources. Traditional optimization approaches encounter complexity due to factors like the large number of cells, stochastic traffic, channel variations, and intricate trade-offs. This paper introduces the simulated reality of communication networks (SRCON) framework, a novel, data-driven modeling paradigm that harnesses live network data and employs a blend of machine learning (ML)- and expert-based models. These mix of models accurately characterizes the functioning of network components, and predicts network energy efficiency and user equipment (UE) quality of service for any energy carrier shutdown configuration in a specific network. Distinguishing itself from existing methods, SRCON eliminates the reliance on expensive expert knowledge, drive testing, or incomplete maps for predicting network performance. This paper details the pipeline employed by SRCON to decompose the large network energy efficiency modeling problem into ML and expert-based submodels. It demonstrates how, by embracing stochasticity, and carefully crafting the relationship between such submodels, the overall computational complexity can be reduced and prediction accuracy enhanced. Results derived from real network data underscore the paradigm shift introduced by SRCON, showcasing significant gains over a state-of-the art method used by a operator for network energy efficiency modeling. The reliability of this local, data-driven modeling of the network proves to be a key asset for network energy-saving optimization.

==> 0X_Table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\centering
\caption{System parameters}
\label{table:parameters}
\def\arraystretch{1.2}
\begin{tabulary}{\columnwidth}{ |p{2.1cm} | p{5.85cm} | }
\hline
	\textbf{TN deployment} 			&  \\ \hline
  Cell layout				& Hexagonal grid over an area $A_{\mathrm{U}} = \SI{52}{km^2}$, $\mathrm{ISD_{TN}} = 500$~m, three sectors per site, one BS per sector at $25$~m   \cite{3GPP36777} \\ \hline
  Frequency band 		& FRF=1, $B_{\nrmx} \!=\!$ 10+10 MHz (DL+UL) at 2~GHz \cite{3GPP36777} \\ \hline
	BS transmit power 			& 46~dBm \cite{3GPP36777} \\ \hline   
	Antenna elements 		& Horiz./vert. HPBW: $65^{\circ}$, max. gain: 8~dBi \cite{3GPP36777} \\ \hline
	Antenna array 		& $10\times 1$, downtilt: $12^{\circ}$, element spacing: $0.5\lambda$ \cite{3GPP36777}\\ \hline
	Noise figure 			& 7~dB \cite{3GPP38901} \\ \hline \hline
	
	\textbf{NTN deployment} 			&  \\ \hline
  Cell layout				& Orbit: 600~km, 7 beams centered on a hexagonal grid, elevation angle: variable \cite{3GPP38821} \\ \hline
  %Frequency band 		& $B_{\nrmx}=$ 30+30 MHz (DL+UL) FDD at 2~GHz \cite{3GPP38821} \\ \hline
  \multirow{2}{*}{Frequency band}		& FRF=1, $B_{\nrmx}\!=\!$ 30+30 MHz (DL+UL) at 2~GHz \cite{3GPP38821}  \\ \cline{2-2} 			& FRF=3, $B_{\nrmx}\!=\!$ 10+10 MHz (DL+UL) at 2~GHz \cite{3GPP38821} \\ \hline
			Transmit power			& 34 dBW/MHz per beam \cite{3GPP38821} \\ \hline
  Beam antenna				& Reflector with circular aperture, HPBW: 4.41$^{\circ}$, max. gain: 30~dBi \cite{3GPP38821} \\ \hline
  $G/T$				& 1.1 dB/K \cite{3GPP38821} \\ \hline\hline

	\textbf{Users} 			&  \\ \hline
  User distribution 				& 15 users per TN sector on average \cite{3GPP36777} \\ \hline
	\multirow{2}{*}{GUE distribution} 				& 80\% indoor, horiz.: uniform, $h_{\rm in}$: uniform in buildings of four to eight floors  \cite{3GPP38901} \\ \cline{2-2}
	 				& 20\% outdoor, horiz.: uniform, $h_{\rm out}=1.5$~m \cite{3GPP38901} \\ \hline
	UAV distribution 				& Outdoor, horiz.: uniform, $h_{\rm UAV}$: 150~m \cite{3GPP36777} \\ \hline
	UAVs/GUEs ratio 				& 3GPP Case~2: 0.7\%, Case~3: 7.1\% \cite{3GPP36777} \\ \hline
	User association				& Based on RSRP (large-scale fading) \\ \hline
	\multirow{2}{*}{Scheduler}		& DL: single-user round robin, $B_k=B_{\nrmx}$  \\ \cline{2-2} %\cite{UbeVilRos2008}
			& UL: multi-user round robin, $B_k=360$~kHz \cite{SedFelLin2020} \\ \hline
		\multirow{2}{*}{UL power control}		& TN: fractional power control with $\alpha = 0.80$, $P_{0} = -85$~dBm, and $P_{\textrm{max}}=23$~dBm \cite{3GPP36777} \\ \cline{2-2} %\cite{UbeVilRos2008}
			& NTN: always max power $P_{\textrm{max}}=23$~dBm \cite{3GPP38821}\\ \hline
	User antenna 		& Omnidirectional, gain: 0~dBi \cite{3GPP36777} \\ \hline
	Noise figure 			& 9~dB \cite{3GPP36777} \\ \hline \hline

	\textbf{Channel model} 			&  \\ \hline
	%Probability of LoS 					& Urban Macro as per \cite{3GPP36777, 3GPP38901,3GPP38811}  \\ \hline
	%Path loss 					& Urban Macro as per \cite{3GPP36777,3GPP38901,3GPP38811}  \\ \hline
	%Shadow fading 		& Urban Macro as per \cite{3GPP36777, 3GPP38901,3GPP38811} \\ \hline
	Large-scale fading 		& Urban Macro as per \cite{3GPP36777, 3GPP38901,3GPP38811} \\ \hline
	\multirow{2}{*}{Small-scale fading}		& TN-GUE: Rayleigh  \\ \cline{2-2} 
			& TN-UAV and NTN-UAV: pure LoS \\ \hline
	Thermal noise 				& -174 dBm/Hz spectral density \cite{3GPP36777}\\ \hline 
	%\textbf{MAC} 			&  \\ \hline
	%Traffic model		& Full buffer \\ \hline
	%\multirow{2}{*}{Scheduler}		& DL: single-user round robin, whole bandwidth  \\ \cline{2-2} %\cite{UbeVilRos2008}
	%		& UL: multi-user round robin, 360~kHz / user \cite{SedFelLin2020} \\ \hline
\end{tabulary}
\vspace{-0.5cm}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{comment}

\begin{table}[!b]
  \begin{center}
    \caption{Simulation parameters for the NTN.}
    \label{tab:NTN table}
    \begin{tabular}{|l|l|} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
    \hline
      \textbf{Parameter} & \textbf{Value}\\
      \hline
      LEO height (\SI{}{\meter}) &  $600 \times 10^3$  \\
      LEO Tx power (\SI{}{dBW/MHz}) &  $34$ \\
      Max. Antenna gain   (\SI{}{\dB}) &  $30$ \\
      $G/T$ (\SI{}{\dB/K}) & $1.1$\\
      Frequency (\SI{}{\GHz}) & $2$\\
      Bandwidth (\SI{}{\MHz}) & $10$ \\
      Outdoor UE percentage & $100$\\
      \hline
    \end{tabular}
  \end{center}
\end{table}

\begin{table}[!b]
  \begin{center}
    \caption{Simulation parameters for the TN.}
    \label{tab:TN table}
    \begin{tabular}{|l|l|} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
    \hline
      \textbf{Parameter} & \textbf{Value}\\
      \hline
      $\ISDs$ (\SI{}{\meter}) & $500$\\
      BS height (\SI{}{\meter}) &  $25$  \\
      BS Tx power (\SI{}{dBm}) &  $46$ \\
      Antenna array configuration & $10\times1$\\
      Antenna down-tilt    & $12^\circ$\\
      Max. Antenna element gain (\SI{}{\dB}) &  $8$ \\
      BS Noise Figure (\SI{}{\dB}) &  $5$ \\
      Frequency (\SI{}{\GHz}) & $2$\\
      Bandwidth (\SI{}{\MHz}) & $10$ \\
      Outdoor UE percentage & $20\%$\\
      Indoor UE percentage & $80\%$\\
      \hline
    \end{tabular}
  \end{center}
  \vspace{-1cm}
\end{table}

\end{comment}

==> 0x_NetworkEnergySavins.tex <==
\section{Network energy saving features}

In this section, 
we review the 3 main network energy saving features available in 5G networks to dynamically minimize energy consumption, 
i.e. symbol, channel and carrier shutdown as well as deep dormancy~\cite{}. 

\subsection{Symbol shutdown}

With symbol shutdown, 
when the BS detects that a downlink symbol carries no data, 
it shuts down the power amplifiers of all its radio frequency (RF) transceivers in real time to reduce the energy consumption.  

This shutdown feature works at a symbol level ---tens of microseconds---, 
and if no UE traffic shaping is applied, 
it does not usually result in any UE performance degradation, 
which is an important characteristic.

Let us note, however,  that the energy savings in this case are opportunistic, 
depending on the traffic arrivals, 
and that the longer the symbol shutdown, the more the energy savings, 
as more circuitry within the amplifiers can be switched off. 
However, due to the 5G signalling design, 
it should be noted that the maximum symbol shutdown time is bounded by the maximum periodicity of the synchronization signal block burst, 160\,ms. 

It should be highlighted that traffic shaping could be used to hold packet or symbol transmissions in the queues to allow for a longer symbol shutdown time at the expense of packet or symbol delay. 

\subsection{Channel shutdown}

With channel shutdown, 
the BS can automatically switch off some MIMO channels during some preset periods.
This is realised by shutting down the power amplifiers of the corresponding RF transceivers. 
For example, a massive MIMO BS with 64 MIMO channels may be reconfigured to operate 32 or 16 MIMO channels, depending on the capacity it has to provide.

This channel shutdown feature works in the order of seconds or minutes, 
and usually, 
it also automatically adjust the common channel transmit power of the cell to ensure that its coverage is maintained.

It should be noted, however, that some coverage or capacity losses may appear when using channel shutdown, 
as the beamforming gain and the number of available MIMO channels in the cell is reduced,
and thus there are less resources to satisfy the camped UEs. 


\subsection{Carrier shutdown}

Carrier shutdown allows for deeper sleeps than symbol and channel shutdown, 
by switching off most of the RF and digital front end components. 

In this case, the cell is usually disconnected for long periods of time, 
tens of minutes or even more. 
This carrier shutdown feature, as a consequence, can result in large energy savings,
but coverage and capacity losses can be significant, 
if carriers are not (de)activated in a coordinated manner across the network.
In more details, some coverage holes may appear when disconnecting a cell,
creating coverage problems, 
if no other cell can provide converge to the UEs of the disconnecting cell. 
Capacity is also affected, 
as a disconnected cell does not allow for the spatial reuse of the spectrum,
and thus the service quality of the UEs of the cells receiving the UEs of the disconnecting cell may be compromised. 
This give rise to an intricate trade-off between network energy consumption and network/UE performance.

\subsection{Deep dormancy}

For completeness, 
let us also mention the feature of dormancy that some products may have, 
which follows a similar logic than carrier shutdown, 
but that additionally also allows to disconnect the base band unit processing. 
This feature provides the deepest sleep and the most energy savings, 
and usually operates in a time frame of hours.  

%\end{comment}



















==> commands.tex <==
% Bold lowercase: syntax \nb# where # is {a ... z, 0,1}
\def\nba{{\mathbf{a}}}
\def\nbb{{\mathbf{b}}}
\def\nbc{{\mathbf{c}}}
\def\nbd{{\mathbf{d}}}
\def\nbe{{\mathbf{e}}}
\def\nbf{{\mathbf{f}}}
\def\nbg{{\mathbf{g}}}
\def\nbh{{\mathbf{h}}}
\def\nbi{{\mathbf{i}}}
\def\nbj{{\mathbf{j}}}
\def\nbk{{\mathbf{k}}}
\def\nbl{{\mathbf{l}}}
\def\nbm{{\mathbf{m}}}
\def\nbn{{\mathbf{n}}}
\def\nbo{{\mathbf{o}}}
\def\nbp{{\mathbf{p}}}
\def\nbq{{\mathbf{q}}}
\def\nbr{{\mathbf{r}}}
\def\nbs{{\mathbf{s}}}
\def\nbt{{\mathbf{t}}}
\def\nbu{{\mathbf{u}}}
\def\nbv{{\mathbf{v}}}
\def\nbw{{\mathbf{w}}}
\def\nbx{{\mathbf{x}}}
\def\nby{{\mathbf{y}}}
\def\nbz{{\mathbf{z}}}
\def\nb0{{\mathbf{0}}}
\def\nb1{{\mathbf{1}}}

% Bold capital letters: syntax \nb# where # is {A ... Z}
\def\nbA{{\mathbf{A}}}
\def\nbB{{\mathbf{B}}}
\def\nbC{{\mathbf{C}}}
\def\nbD{{\mathbf{D}}}
\def\nbE{{\mathbf{E}}}
\def\nbF{{\mathbf{F}}}
\def\nbG{{\mathbf{G}}}
\def\nbH{{\mathbf{H}}}
\def\nbI{{\mathbf{I}}}
\def\nbJ{{\mathbf{J}}}
\def\nbK{{\mathbf{K}}}
\def\nbL{{\mathbf{L}}}
\def\nbM{{\mathbf{M}}}
\def\nbN{{\mathbf{N}}}
\def\nbO{{\mathbf{O}}}
\def\nbP{{\mathbf{P}}}
\def\nbQ{{\mathbf{Q}}}
\def\nbR{{\mathbf{R}}}
\def\nbS{{\mathbf{S}}}
\def\nbT{{\mathbf{T}}}
\def\nbU{{\mathbf{U}}}
\def\nbV{{\mathbf{V}}}
\def\nbW{{\mathbf{W}}}
\def\nbX{{\mathbf{X}}}
\def\nbY{{\mathbf{Y}}}
\def\nbZ{{\mathbf{Z}}}

\def\nbtheta{\boldsymbol{\theta}}
\def\nbphi{\boldsymbol{\phi}}

% Serif lowercase: syntax \nsf# where # is {a ... z, 0,1}
\def\nsfa{{\mathsf{a}}}
\def\nsfb{{\mathsf{b}}}
\def\nsfc{{\mathsf{c}}}
\def\nsfd{{\mathsf{d}}}
\def\nsfe{{\mathbf{e}}}
\def\nsff{{\mathbf{f}}}
\def\nsfg{{\mathbf{g}}}
\def\nsfh{{\mathbf{h}}}
\def\nsfi{{\mathbf{i}}}
\def\nsfj{{\mathbf{j}}}
\def\nsfk{{\mathbf{k}}}
\def\nsfl{{\mathbf{l}}}
\def\nsfm{{\mathbf{m}}}
\def\nsfn{{\mathbf{n}}}
\def\nsfo{{\mathbf{o}}}
\def\nsfp{{\mathbf{p}}}
\def\nsfq{{\mathbf{q}}}
\def\nsfr{{\mathbf{r}}}
\def\nsfs{{\mathbf{s}}}
\def\nsft{{\mathbf{t}}}
\def\nsfu{{\mathbf{u}}}
\def\nsfv{{\mathbf{v}}}
\def\nsfw{{\mathbf{w}}}
\def\nsfx{{\mathbf{x}}}
\def\nsfy{{\mathbf{y}}}
\def\nsfz{{\mathbf{z}}}

% Serif lower letters: syntax \nsf# where # is {A ... Z}
\def\nsfA{{\mathsf{A}}}
\def\nsfB{{\mathsf{B}}}
\def\nsfC{{\mathsf{C}}}
\def\nsfD{{\mathsf{D}}}
\def\nsfE{{\mathsf{E}}}
\def\nsfF{{\mathsf{F}}}
\def\nsfG{{\mathsf{G}}}
\def\nsfH{{\mathsf{H}}}
\def\nsfI{{\mathsf{I}}}
\def\nsfJ{{\mathsf{J}}}
\def\nsfK{{\mathsf{K}}}
\def\nsfL{{\mathsf{L}}}
\def\nsfM{{\mathsf{M}}}
\def\nsfN{{\mathsf{N}}}
\def\nsfO{{\mathsf{O}}}
\def\nsfP{{\mathsf{P}}}
\def\nsfQ{{\mathsf{Q}}}
\def\nsfR{{\mathsf{R}}}
\def\nsfS{{\mathsf{S}}}
\def\nsfT{{\mathsf{T}}}
\def\nsfU{{\mathsf{U}}}
\def\nsfV{{\mathsf{V}}}
\def\nsfW{{\mathsf{W}}}
\def\nsfX{{\mathsf{X}}}
\def\nsfY{{\mathsf{Y}}}
\def\nsfZ{{\mathsf{Z}}}

\def\nsfTheta{\mathsf{\Theta}}
\def\nbphi{\boldsymbol{\phi}}

% \mathcal: syntax \ncal# where # is {A ... Z}
\def\ncalA{{\mathcal{A}}}
\def\ncalB{{\mathcal{B}}}
\def\ncalC{{\mathcal{C}}}
\def\ncalD{{\mathcal{D}}}
\def\ncalE{{\mathcal{E}}}
\def\ncalF{{\mathcal{F}}}
\def\ncalG{{\mathcal{G}}}
\def\ncalH{{\mathcal{H}}}
\def\ncalI{{\mathcal{I}}}
\def\ncalJ{{\mathcal{J}}}
\def\ncalK{{\mathcal{K}}}
\def\ncalL{{\mathcal{L}}}
\def\ncalM{{\mathcal{M}}}
\def\ncalN{{\mathcal{N}}}
\def\ncalO{{\mathcal{O}}}
\def\ncalP{{\mathcal{P}}}
\def\ncalQ{{\mathcal{Q}}}
\def\ncalR{{\mathcal{R}}}
\def\ncalS{{\mathcal{S}}}
\def\ncalT{{\mathcal{T}}}
\def\ncalU{{\mathcal{U}}}
\def\ncalV{{\mathcal{V}}}
\def\ncalW{{\mathcal{W}}}
\def\ncalX{{\mathcal{X}}}
\def\ncalY{{\mathcal{Y}}}
\def\ncalZ{{\mathcal{Z}}}

% \mathbb: syntax \nbb# where # is {A ... Z}
\def\nbbA{{\mathbb{A}}}
\def\nbbB{{\mathbb{B}}}
\def\nbbC{{\mathbb{C}}}
\def\nbbD{{\mathbb{D}}}
\def\nbbE{{\mathbb{E}}}
\def\nbbF{{\mathbb{F}}}
\def\nbbG{{\mathbb{G}}}
\def\nbbH{{\mathbb{H}}}
\def\nbbI{{\mathbb{I}}}
\def\nbbJ{{\mathbb{J}}}
\def\nbbK{{\mathbb{K}}}
\def\nbbL{{\mathbb{L}}}
\def\nbbM{{\mathbb{M}}}
\def\nbbN{{\mathbb{N}}}
\def\nbbO{{\mathbb{O}}}
\def\nbbP{{\mathbb{P}}}
\def\nbbQ{{\mathbb{Q}}}
\def\nbbR{{\mathbb{R}}}
\def\nbbS{{\mathbb{S}}}
\def\nbbT{{\mathbb{T}}}
\def\nbbU{{\mathbb{U}}}
\def\nbbV{{\mathbb{V}}}
\def\nbbW{{\mathbb{W}}}
\def\nbbX{{\mathbb{X}}}
\def\nbbY{{\mathbb{Y}}}
\def\nbbZ{{\mathbb{Z}}}

% \mathfrak:
\def\nfrakR{{\mathfrak{R}}}

% Roman: {\rm } syntax \nrm# where # is {a ... z}
\def\nrma{{\rm a}}
\def\nrmb{{\rm b}}
\def\nrmc{{\rm c}}
\def\nrmd{{\rm d}}
\def\nrme{{\rm e}}
\def\nrmf{{\rm f}}
\def\nrmg{{\rm g}}
\def\nrmh{{\rm h}}
\def\nrmi{{\rm i}}
\def\nrmj{{\rm j}}
\def\nrmk{{\rm k}}
\def\nrml{{\rm l}}
\def\nrmm{{\rm m}}
\def\nrmn{{\rm n}}
\def\nrmo{{\rm o}}
\def\nrmp{{\rm p}}
\def\nrmq{{\rm q}}
\def\nrmr{{\rm r}}
\def\nrms{{\rm s}}
\def\nrmt{{\rm t}}
\def\nrmu{{\rm u}}
\def\nrmv{{\rm v}}
\def\nrmw{{\rm w}}
\def\nrmx{{\rm x}}
\def\nrmy{{\rm y}}
\def\nrmz{{\rm z}}

% Hat characters
\def\hatgamma{\widehat{\gamma}}



% Special symbols
\def\nbydef{:=}
\def\nborel{\ncalB(\nbbR)}
\def\nboreld{\ncalB(\nbbR^d)}
\def\sinc{{\rm sinc}}

% Theorems etc.
\newtheorem{lemma}{Lemma}
\newtheorem{thm}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{ndef}{Definition}
\newtheorem{nrem}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{cor}{Corollary}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}
\newtheorem{approximation}{Approximation}
	
%%%%%%%% Backwards compatibility

\newcommand{\ceil}[1]{\lceil #1\rceil}
\def\argmin{\operatorname{arg~min}}
\def\argmax{\operatorname{arg~max}}
\def\figref#1{Fig.\,\ref{#1}}%
\def\E{\mathbb{E}}
\def\EE{\mathbb{E}^{!o}}
\def\P{\mathbb{P}}
\def\pc{\mathtt{P_c}}
\def\rc{\mathtt{R_c}}   % rate coverage
\def\p{p}
\def\ie{{\em i.e.}}
\def\eg{{\em e.g.}}
\def\V{\operatorname{Var}}
\def\erfc{\operatorname{erfc}}
\def\erf{\operatorname{erf}}
\def\opt{\mathrm{opt}}
\def\R{\mathbb{R}}
\def\Z{\mathbb{Z}}

\def\LL{\mathcal{L}^{!o}}
\def\var{\operatorname{var}}
\def\supp{\operatorname{supp}}

\def\N{\sigma^2}
\def\T{\beta}							% Threshold = \beta_i
\def\sinr{\mathtt{SINR}}			% Signal to interference plus noise ratio
\def\snr{\mathtt{SNR}}
\def\sir{\mathtt{SIR}}
\def\ase{\mathtt{ASE}}
\def\se{\mathtt{SE}}

\def\calN{\mathcal{N}}
\def\FE{\mathcal{F}}
\def\calA{\mathcal{A}}
\def\calK{\mathcal{K}}
\def\calT{\mathcal{T}}
\def\calB{\mathcal{B}}
\def\calE{\mathcal{E}}
\def\calP{\mathcal{P}}
\def\calL{\mathcal{L}}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Pois}{Pois}

\def\R{{\mathbb{R}}}
\def\C{{\mathbb{C}}}
\newcommand{\tran}{^{\text{\sf T}}}
\newcommand{\herm}{^{\text{\sf H}}}

